Co-evolution of language and agents in referential games

Referential games offer a grounded learning environment for neural agents which accounts for the fact that language is functionally used to communicate. However, they do not take into account a second constraint considered to be fundamental for the shape of human language: that it must be learnable by new language learners. Cogswell et al. (2019) introduced cultural transmission within referential games through a changing population of agents to constrain the emerging language to be learnable. However, the resulting languages remain inherently biased by the agents' underlying capabilities. In this work, we introduce Language Transmission Engine to model both cultural and architectural evolution in a population of agents. As our core contribution, we empirically show that the optimal situation is to take into account also the learning biases of the language learners and thus let language and agents co-evolve. When we allow the agent population to evolve through architectural evolution, we achieve across the board improvements on all considered metrics and surpass the gains made with cultural transmission. These results stress the importance of studying the underlying agent architecture and pave the way to investigate the co-evolution of language and agent in language emergence studies.

==> evolving_networks copy/abstract.tex <==
\begin{abstract}
%\dieuwke{Rewrite abstract at the end}
Referential games offer a grounded learning environment for neural agents which accounts for the fact that language is functionally used to communicate.
However, they do not take into account a second constraint considered to be fundamental for the shape of human language: that it must be learnable by new language learners. % and thus has to overcome a \textit{transmission bottleneck}.

\citet{Cogswell2019} introduced \emph{cultural transmission} within referential games through a changing population of agents to constrain the emerging language to be learnable.
However, the resulting languages remain inherently biased by the agents' underlying capabilities. 

In this work, we introduce \ourframework~to model both cultural and architectural evolution in a population of agents.
%We find supporting evidence that the introduction of \emph{cultural transmission} results in a substantial improvement in language efficiency and communicative success. 
As our core contribution, we empirically show that the optimal situation is to take into account also the learning biases of the language learners and thus let language and agents \textit{co-evolve}.
When we allow the agent population to evolve through architectural evolution, we achieve across the board improvements on all considered metrics and surpass the gains made with \emph{cultural transmission}.
These results stress the importance of studying the underlying agent architecture and pave the way to investigate the \textit{co-evolution} of language and agent in language emergence studies.

%In this work, we introduce this \emph{cultural transmission} component in a referential game, by introducing a changing population of agents in which new agents learn by playing with more experienced agents, and show that the introduction of such \emph{cultural transmission} results in a substantial improvement in language efficiency and communicative success. %, measured in convergence speed, degree of structure in the emerged languages and within-population consistency of the language.
%However, as our core contribution, we show that the optimal situation is to take into account also the learning biases of the language learners and thus let language and agents \textit{co-evolve}: when we allow the agent population to evolve through architectural evolution, we achieve across the board improvements on all considered metrics.
%These results stress that for language emergence studies \textit{cultural evolution} is important, but also the suitability of the architecture itself should be considered. 
% % However, they do not consider a second constraint to be fundamental for the shape of human language: that it has to overcome a \textit{transmission bottleneck} because it must be learnable by new language users.
% % Crucially, the inputs to this game are compositionally generated images that would be described well by a compositional language.
% % Interestingly, senders and receivers evolve into different architectures, which prove to be more effective at the referential game than standard LSTMs.
% %, and with this paves the way for investigating the emergence of language with more natural pressures.
%  % We then offer two ways to deal with it: adapting the language to accommodate the bottleneck via cultural evolution or changing the bottleneck by evolving agents' genotypical design. 
% % We show how co-evolving cultural and genetic adaptations is crucial for achieving the most efficient language transmission (how quickly newbies master communication) as well as more interesting structural properties of the language (how compositional is the emergent language). 
\end{abstract}


==> evolving_networks copy/acknowledgments.tex <==
\section{Acknowledgements}
\label{sec:acknowledgements}
We would like to thank Angeliki Lazaridou for her helpful discussions and feedback on previous iterations of this work.



==> evolving_networks copy/analysis.tex <==
\section{Analysis}

% \dieuwke{Explain what we do here}

In this section we analyse the resulting behaviour and success of agents in \ourframework.
We first use standard approaches such as average agent entropy and loss (convergence) to measure the success of agents with respect to their language and the task. 
Secondly, we use other metrics to analyse the emergent language itself in terms of consistency and diversity by using Jaccard Similarity, the proportion of unique matches, the number of unique messages, and the topographic similarity.
Thirdly, we perform a qualitative analysis of the architecture that emerge from our \ourframework.
Finally, we design Frozen Experiments, in which we test the emerged languages and architectures in a 1v1 setting with a fresh agent. 
This allows us to compare and measure the the improvement gains made by the architecture and those made by the language which emerged.
We show through these experiments that the co-evolution setting leads to a language that is both more successful and easier to learn for a given new agent. 

\subsection{Agent behaviour}

To assess the behaviour of the agents over time, we monitor their average message entropy convergence speed.
As can be seen in Figure~\ref{fig:ent}, the \texttt{\normalsize co-evolution} setup results in the lowest average entropy scores, the messages that they assign to one particular image will thus have lower variation than in the other setups.
Of the cultural evolution setups, the lowest entropy score is achieved in the \texttt{cu-best} setup.
% Interestingly, the average message entropy in both these setups appears to still go down, long after many of the other metrics have converged.

\begin{figure}[h!]
	\centering
	\includegraphics[width=\columnwidth, trim = 14mm 0mm 20mm 10mm]{images/run_images/entropy}
	\caption{Average agent entropy over time.}
	\label{fig:ent}
\end{figure}

Figure \ref{fig:convergence} shows the average population convergence over time. 
Also in this case, we observe a clear difference between cultural evolution only and co-evolution, with an immediately much lower convergence time for co-evolution and a slightly downward trending curve. 
% maybe some of the models not often getting refreshed and so they can attain very low entropy?

\begin{figure}[h!]
	\centering
	\includegraphics[width=\columnwidth, trim= 14mm 0mm 20mm 10mm, clip]{images/run_images/avg_convergence}
	\caption{Average convergence for all cultural transmission modes and evolution.}
	\label{fig:convergence}
\end{figure}

%\textcolor{gray}{New agents added to a population with low convergence should be faster learners than if they were added to a population with a higher convergence.}

%\textcolor{red}{While these results are clearly in favour of evolution, they do not necessarily translate to higher average accuracy on the task.
%%% @TODO Add reasons here
%This is for the simple reason that each measurement is taken after} 
%This is not reflected in the accuracy for 


%% extra analysis : 
\subsection{Language Analysis}
%analysis of the emerging languages

\begin{figure}[h]
	\includegraphics[width=\columnwidth, trim = 19mm 0 20mm 15mm, clip]{images/run_images/similarity}
	\caption{Average Jaccard Similarity and proportion of message matches for all cultural transmission modes and evolution}
	\label{fig:similarity}
\end{figure}

%EXPAND
To check the consistencies of languages within a population, we compare the Jaccard Similarity and the Average Proportion of Unique Matches, which we plot in Figure \ref{fig:similarity}. This shows that, compared to cultural evolution only, not only are the messages in co-evolution more similar across agents (higher Jaccard Similarity), but also that agents are considerably more aligned with respect to the same inputs (less unique matches). 

\begin{figure}[h]
	\includegraphics[width=\columnwidth, trim = 13mm 0 2mm 21mm, clip]{images/run_images/topo_unique}
	\caption{Average Number of Unique Messages and Topographic Similarity for all cultural evolution modes and co-evolution.
        For comparison, we also plot the number of unique messages for a symbolic solution that fully encodes all relevant features of the image (since we have three possible shapes and colours, two possible sizes, and a $3 \times 3$ grid of possible positions, this symbolic reference solution has $3 \times 3 \times 2 \times 9 = 162$ distinct messages.}
	\label{fig:topo}
\end{figure}

%It is also possible that this effect is partly due to a smaller usage of unique messages by the population.

To assess the level of structure of the emerged languages, 
we plot the average Topographic Similarity and the Average Number of Unique Messages generated by all senders (Figure \ref{fig:topo}). 
The co-evolution condition again outperforms all cultural only conditions, with a simpler language (the number of the unique messages closer to the symbolic reference point) that is structurally more similar to the symbolic representation of the input (higher Topographical Similarity). 
% For the unique messages, we show also the `optimal' solution when the input is fully described using the original symbolic representation.\footnote{
%From these results, we note the relationship between the two measures, where a simpler language which will 
%the black line in the minimum number of messages describes the minimum messages needed to describe the input space using the symbolic calculation. 
%\textcolor{red}{However it is important to note that this solution is insufficient to solve the task using image features extracted from raw images, because there are perturbations in the location of objects in the grid pixel space. It is possible that two images with the same symbolic representations have slightly different pixels since the object can be positioned in a range of different positions within the same symbolic position.} 

\subsection{Architecture Analysis}
\label{sec:arch_analysis}
%analysis of the found architecture on the task

\begin{figure*}[h!]
	\centering
	\includegraphics[width=\textwidth]{images/qualitative_analysis.png}
	\caption{Evolution of the best sender and receiver architecture according to convergence, and the evolution of the population's message description of the same input through iterations. 
	The bold messages represent the message outputted by the best sender whose architecture is pictured above. 
	The count of each message represents the number of agents in the population which uttered this exact sequence. }
	\label{fig:qualitative}
\end{figure*}

In Figure \ref{fig:qualitative} we show the co-evolution of an agent and a sample of its language during three selected iterations in the co-evolution setup.
Strikingly, the best sender architecture does not evolve from its original form, which could point towards the limitations of of our search strategy and space.
% language to describe an image in the data set during three selected iterations from the co-evolution setup.
% The best sender and receiver architectures according to convergence are shown above and below the messages respectively.
% The messages are ordered by most uttered and the number following each line counts the number of agents which generated the same message. 
% The bold message indicates that it was uttered by the best sender architecture.
% In this case we observe that the best sender architecture does not evolve from its original form, and could point towards the limitations of using such a simple evolution strategies. 
% Since no model one edit step away is better than this architecture in terms of convergence, the evolution is probably unable to get out of the local optima.
On the contrary, the receiver goes through quite some evolution steps and converges into a significantly more complex architecture than its original form.
We observe a unification of language throughout evolution in Figure \ref{fig:qualitative}, which is also supported by Figure \ref{fig:topo}. 
The population of senders starts out 11 different unique messages and ends with only two to describe the same input image. 
We will leave more detailed analysis of the evolved architectures for future work.

\subsection{Frozen Experiments}

With a series of experiments we test the a priori suitability of the evolved languages and agents for the task at hand, by monitoring the accuracy of new agents that are paired with converged agents and train them from scratch.

We focus, in particular, on training receivers with a frozen sender from different setups, which allows us to assess 1) whether cultural evolution made languages evolve to be more easily picked up by new agents 2) whether the genetic evolution made architectures converge more quickly when faced with this task.
We compare the accuracy development of:\begin{itemize}
    \item An LSTM receiver trained with a frozen sender taken from \texttt{cu-best};
    \item An evolved receiver trained with a frozen evolved sender.
\end{itemize}
For both these experiments, we compare with two baselines:\begin{itemize}
    \item The performance of a receiver agent trained from scratch along with a receiver agent that has either the \texttt{cu} architecture or the evolved \texttt{co} architecture (\texttt{cu-baseline} and \texttt{co-baseline}, respectively);
    \item The performance of an agent trained with an agent that is \textit{pretrained} in the single agent setup, with either the \texttt{cu} architecture or an evolved architecture (\texttt{\normalsize cu-baseline-pretrained} and \texttt{co-baseline-pretrained}).
\end{itemize}

Each experiment is run 10 times, keeping the same frozen agent.
The results confirm cultural evolution contributes to the learnability and suitability of emerging languages: the \texttt{cu-best} accuracy (green line) converges substantially quicker and is substantially higher than the \texttt{cu-baseline-pretrained} accuracy (orange line). 
Selective pressure on the language appears to be important: the resulting languages are only easier to learn in the \texttt{cu-best} setup.\footnote{\texttt{cu-age} and \texttt{cu-random} are ommitted from the plot for clarity reasons.}
%TODO say something about selection?
In addition, they show that the agents benefit also from the genetic evolution: the best accuracies are achieved in the co-evolution setup (red line).
The difference between the \texttt{cu-baseline} (blue) and the \texttt{co-baseline} (brown) further shows that even if the evolved architectures are trained from scratch, they perform much better than a baseline model trained from scratch.
The difference between the \texttt{co-baseline-pretrained} (only genetic evolution, purple line) and the co-evolution of agents and language line (red line) illustrates that genetic evolution alone is not enough: while a new evolved receiver certainly benefits from learning from a (from scratch) pretrained evolved sender, without the cultural transmission pressure, it's performance is still substantially below a receiver that learns from an evolved sender whose language was evolved as well.

\begin{figure}
	\includegraphics[width=\columnwidth, trim = 12mm 0 13mm 15mm, clip]{images/frozen_images/frozen_senders.png}
	\caption{Receiver accuracies trained with different types of frozen senders.}
	\label{fig:frozen_sender}
\end{figure}

% While also the reverse experiment -- teaching a Sender agent with a frozen receiver agent -- could be done, these results are less

%This pre-trained model is trained for 10,000 iterations and the best model during training is selected based on validation accuracy.
%The pre-trained baseline as a result has a very specialized language with numerous unique words since it is trained with a single opposing receiver.
% We note that the accuracy and speed of the learning is more superior with pre-training with a frozen sender than with learning from scratch.

% The specify the evolution baseline (`e\_baseline') as the case where the best sender architecture found and the best receiver architecture found through evolution are trained from scratch in a two-agent-setting.
% Its pre-trained version (`e\_baseline\_pretrained') takes a frozen pre-trained evolved sender and pairs it with an evolved receiver. 
% The difference between the `baseline' and the 'e\_baseline' curves can be interpreted as part of the impact of neural evolution on convergence.

% Now looking at the cultural evolution (\textbf{best}, \textbf{age}, \textbf{random}) and LTE (\textbf{evolution}) results, Figure \ref{fig:frozen_sender} shows the impact of language on not only faster but also more successful learning.

% These results further demonstrate that average population accuracy is not enough to understand the quality of the language in a population since it is affected directly by culling.
% When culling is removed and we compare the multi-agent approaches back into a two-agent setting, we can observe these methods to outshine any naive two-agent approaches.

% \begin{figure}[h]
% 	\includegraphics[width=0.5\textwidth]{images/frozen_images/frozen_receivers.png}
% 	\caption{Accuracy for frozen receivers (e for evolved sender architecture)}
% 	\label{fig:frozen_receivers}
% \end{figure}
% 
% In Figure \ref{fig:frozen_receivers}, we show the results of the reverse experiments, in which we use a frozen receiver to teach a new sender model.
% The results of these experiments
% 
% In this case, the 'baseline' training from scratch fares much better, being on par with cultural evolution (\textbf{age}, \textbf{random}). 
% The orange line shows that pre-training on the baseline task does not improve it and in facts, makes it worse. 
% This indicates that it is harder for the sender to learn from a frozen receiver than the reverse.
% Therefore the pre-trained receiver which understands a complex language fails to teach it to the sender. 
% This relationship also seems to happen, albeit less so, with the cultural evolution \textbf{best}.
% 
% Using frozen receivers in Figure \ref{fig:frozen_receivers}, we also note the three evolution based methods outperforming the rest.
% 







==> evolving_networks copy/approach.tex <==
\section{Approach}
\label{sec:approach}
%\dieuwke{These sentences should probably be rephrased, content should be something like this though:} 
In this paper, we introduce architectural evolution in language emergence games and study the interaction between cultural and architectural evolution with a range of different metrics.
Below, we first give a definition of the referential game we consider (Subsection~\ref{sec:referential_game}).
We then briefly explain our \ourframework~(Section ~\ref{sec:ourframework} and how we model cultural and architectural evolution within it ~(Section \ref{sec:cuevo} and \ref{sec:archevo} respectively).
%The most substantial part of our contributions is described in Section \ref{sec:archevo}, in which we introduce architectural evolution.

\subsection{Referential games}\label{sec:referential_game}
%\dieuwke{Shorten this a bit}
We study language emergence in a referential game inspired by the signalling games proposed by \citet{lewis1969convention}.
In this game, one agent (the \textit{sender}) observes an image and generates a discrete message.
The other agent (the \textit{receiver}) uses the message to select the right image from a set of images containing both the sender image and several distractor images.
Since the information shown to the sender agent is crucial to the receivers success, this setup urges the two agents to come up with a communication protocol that conveys the right information.

Formally, our \textit{referential} game is similar to \citet{Havrylov2017}: %  and \citet{Choi2018}:
{\small \begin{enumerate}[itemsep=-1ex]
    \item The meaning space of the game consists of a collection $D$ of $K$ images $\{d_0,d_1, ..., d_K\}$, represented by $z$-dimensional feature vectors.
    \item In each round $i$ of the game, a target item $d_i$ is randomly sampled from $D$, along with a set $C$ of $n$ distractor items.
    \item The sender agent $s$ of the game, parametrised by a neural network, is given item $d_i$, and generates a discrete message $m_i$ from a vocabulary $V$.
The message is capped to a max message length of $L$.
    \item The receiver agent $r$, also parametrised by a neural network, receives message $m_i$ and uses it to identify $d_i$ in the union of $d_i$ and $C$.
\end{enumerate}
}
\noindent We use $z=512$, and $n=3$ and train agents with Gumbel-Softmax \cite{jang2017categorical} based on task-success.

% \begin{enumerate}
% 	\item A collection $D$ of $N$ items $\{d_0,d_1, ..., d_N\}$, a sender agent $s$ and a receiver agent $r$;
% 	\item A target item $d_i$, sampled randomly from the $D$, along with a subset $C \subset D$ of $\delta$ distractor items;
% 	\item Sender $s$ is shown item $d_i$, generates a discrete message $m_i$ from a vocabulary $V$ of size $|V|$. 
% 	The message is capped to a max sentence length of size $l$. 
% 	\item Receiver $r$ receives message $m_i$ as input.
% 	\item We test with $\delta=4$ and $d_i \in C$: Receiver $r$ picks item $d_i$ out of collection $C$.
% \end{enumerate}

%ST Gumbel-Softmax has been used successfully in the context of multi-agent communication before \cite{Havrylov2017}, and allows us to bypass the traditional reinforcement learning approaches for a faster training.
%Using such a trick also allows us have a single training regime, rather than alternating sender and receiver agents as in \citet{Choi2018}. 
%
%The potential downside of using Gumbel-Softmax is that during training time agents could learn to communicate through none discrete messages, thus effectively removing any bottleneck that we seek to enforce.
%However,  since we find no decrease in accuracy on tasks when evaluating and using the discrete outputs to make predictions on validation sets, we do not find this to be a problem. 

\subsection{\ourframework}
\label{sec:ourframework}
In \ourframework, depicted in Figure~\ref{fig:lte}, we simulate a population of communicating agents.
In every training iteration, two random agents are sampled to play the game.
This forces the agents to adopt a simpler language naturally: to succeed they must be able to communicate or understand all opposing agents.
In our setup, agents are either sender or receiver, they do not switch roles during their lifetime.

\subsection{Cultural evolution in referential games}
\label{sec:cuevo}
Following \citet{Cogswell2019}, we simulate cultural evolution by periodically replacing agents in the population with newly initialised agents.
Cultural evolution is implicitly modelled in this setup, as new agents have to learn to communicate with agents that already master the task.
Following \citet{Cogswell2019}, we experiment with three different methods to select the agents that are replaced: randomly (no selection pressure), replacing the oldest agents or replacing the agents with the lowest fitness (as defined in Section~\ref{sec:fitness}).
We call these setups \texttt{cu-random}, \texttt{cu-age} and \texttt{cu-best}, respectively.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{images/CEE}
	\caption{The \ourframework: Agent pairs are randomly sampled from each population and trained. After $l$ training steps, a portion $\alpha$ of the population is culled.}
	\label{fig:lte}
\end{figure}


\subsection{Architectural evolution in referential games}
\label{sec:archevo}
%\dieuwke{Some of the text from the previous related work might need to be mentioned here, I copied it to text\_related\_work\_prev\_stored.tex}
% Gautier: Added some back

% Though it is important to note that simply increasing the population size would not lead to true cultural transmission pressure, since the emergent language would eventually grow in complexity as every agent starts to learn it and knows that every other agents speaks the same. 
% \citet{Cogswell2019}, create a knowledge gap by re-initialising a subset of agents periodically  in order to force compression of the language through cultural transmission.
% Therefore it is the uncertainty of agents about the language of their partners, rather than the sheer number of them, which drives the cultural transmission and subsequent compressibility pressure. 
% Cultural evolution is implicitly modelled in this setup, as new agents have to learn to communicate with agents that already master the task.

To model architectural evolution, rather than periodically replacing agents with randomly initialised new agents, we instead mutate the most successful agents and replace the worst agents with variations of the best agents, as outlined in Section~\ref{sec:mutation}.
Note that cultural evolution is still implicitly modelled in this setup, as new agents still have to learn to communicate with older agents.
Therefore, we call this setup with the term \texttt{co-evolution}.


\subsubsection{Culling} We refer to the selection process and subsequent mutation or re-initialisation step as \textit{culling}. 
% The fitness-based evolutionary pressure leads our populations to capture part of the inherent biases of language within the neural architecture and thus promote faster learners on the task. 
% Mutating agents forces language to remain simpler and general, but also encourages fast learners in a sort of meta-learning approach. 
In biology, culling is the process of artificially removing organisms from a group to promote certain characteristics, so, in this case, culling consists of removing a subset of the worst agents and replacing them with variations of the best architecture.
The proportion of agents from each population selected to be mutated is determined by the culling rate $\alpha$, where $\alpha \in [0, 1)$.
The culling interval $l$ defines the number of iterations between culling steps.
A formalisation of the LTE can be found in appendix~\ref{app:lte}.

\subsubsection{Mutation Algorithm}\label{sec:mutation}
\label{sec:mutation_algo}
% [Approx one column]

Our mutation algorithm is an intentionally simple implementation of a Neural Architectural Search (NAS).
NAS focuses on searching the architecture space of networks, unlike many traditional evolutionary techniques which often include parameter weights in their search space.
We opted to use the DARTS (Differentiable Architecture Search) RNN search space defined by  \citet{Liu2018}, which has obtained state-of-the-art performance on benchmark natural language tasks \cite{Li2019}.

The DARTS search space includes recurrent cells with up to $N$ nodes, where each node $n_1, n_2,...,n_N$ can take the output of any preceding nodes including $n_0$, which represents the cell's input.
All potential connections are modulated by an activation function, which can be the identity function, Tanh, Sigmoid or ReLU.
Following \citet{Liu2018} and \citet{Pham2018}, we enhance each operation with a highway bypass \cite{Zilly2016} and the average of all intermediate nodes is treated as the cell output.

To sample the initial model, we sample a random cell with a single node ($N=1$).
As this node must necessarily be connected to the input, the only variation stems from the possible activation functions applied to the output of $n_1$, resulting in four possible starting configurations.
We set a node cap of $N=8$.
% We initialise our evolution with $N=1$ and set a node cap to $N=8$. %, reducing the initial search space and encouraging a simpler structure.
We mutate cells by randomly sampling an architecture which is one edit step away from the previous architecture.
Edit steps are uniformly sampled from i) changing an incoming connection, ii) changing an output operation or iii) adding a new node; the mutation location is uniformly sample from all possible mutations.\footnote{For a formal description of the mutation process, we refer to Appendix~\ref{app:mutation}.}
% Each new mutated network is initialised with random weights.
%Note that while we use the DARTS search space to define potential mutations, contrary to \citet{Liu2018}, we do not use differentation to sample new architectures based on a selection criterion.

\subsection{Fitness Criterion}
\label{sec:fitness}

The fitness criterion that we use in both the \texttt{cu-best} and \texttt{co-evolution} setup is based on task performance.
However, rather than considering agents' performance right before the culling step, we consider the age of the youngest agent in the population (defined in terms of number of batches that it was trained) and for every agent compute their performance up until \textit{when they had that age}.
For any agent $a_j$ in population $\mathbf{A}$ this is defined as: 
\begin{equation}
    \text{fitness}(a_j)= \frac{1}{\mathcal{T}_A}\sum_{t=0}^{\mathcal{T}_A} \mathcal{L}(a_j^t)
\end{equation}
where $\mathcal{T}_A = \min_{a \in A}\mathcal{T}(a)$ is the age $\mathcal{T}(a)$  of the youngest agent in the population, and $\mathcal{L}(a_j^t)$ is the loss of agent $a_j$ at time step $t$.
This fitness criterion is not biased towards older agents, that have seem already more data and have simply converged more.
It is thus not only considering task performance but also the \textit{speed} at which this performance is reached.

% We propose \textit{convergence} as a metric which describes how fast an agent picks up the language in comparison to others, and use it in the selection process.
% Convergence allows us to test whether language becomes simpler through cultural transmission as it should pressure the language to be simpler. 

%We mutate the best genotype in order to replace the worst $\alpha$ proportion of agents according to convergence with these new variations. 

% Where $min(age(A))$ is the minimum age out of all agents in the population, $loss_{j,t}$ is the batch loss of the agent at age $t$, and age is calculated as the number of batches seen.
% We only average over the minimum number of batches seen, in order not to bias towards older agents which might have seen more data and converged. 
%Since we only re-initialise a sub-population of agents periodically, the maximum age in the population can vary greatly and affect the results of a naive historical loss average.

%Therefore we can view this fitness criterion and evolutionary process as a system of meta-learning or learning to learn, in which agents that learn the fastest will amount to lower convergence.

% We also use this convergence metric in order to select the worst agents to re-initialise in cultural transmission when testing a greedy sampling and $\argmax$ approach.  




==> evolving_networks copy/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we introduced a language transmission bottleneck in a referential game, where new agents have to learn the language by playing with more experienced agents. 
To overcome such bottleneck, we enabled both the cultural evolution of language and the architectural evolution of agents, using a new \ourframework. 
Using a battery of metrics, we monitored their respective impact on communication efficiency, degree of linguistic structure and intra-population language homogeneity. While we could find important differences in between cultural evolution strategies, it is when we included architectural evolution that agents scored best.
In a second experiment, we paired new agents with evolved languages and agents and again confirmed that, while cultural evolution makes a language easier to learn, co-evolution leads to the best communication.  

In future research, we would like to apply the \ourframework~on new, more complex tasks and further increase our understanding of the properties of the emerged languages and architectures.
Recent research has also found that relaxing the vocabulary size $V$ and sequence length $L$ constraints can lead to greater syntactic structure in emergent languages \cite{van-der-wal-etal-2020-grammar}.
We thus hope to investigate further relaxation of hyper-parameters and other neuro-evolution techniques in future work.

%For future work: 
%- Smoothing out mutation rate (mutate very often first, then less and less)


==> evolving_networks copy/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

%Introduce datasets
%frame section 

We test the LTE framework on a compositionally defined image dataset, using a range of different selection mechanisms.

% Metrics: of course, task success; but also specific metrics to keep track of evolution, such as (i) speed of task learning (and, consequentially, language learning); metrics on language similarity across agents; metrics to indicate level of linguistic structure; compositionality; something to check if low-level patterns are captured; causal influence?
 
\subsection{Dataset}
\label{subsec:dataset}
In all our experiments, we use a modified version of the Shapes dataset \cite{Andreas2015}, which consists of 30 by 30 pixel images of 2D objects, characterised by shape (circle, square, triangle), colour (red, green, blue), and size (small, big). 
While every image has a unique symbolic description -- consisting of the shape, colour and size of the object and its horizontal and vertical position in a 3x3 grid -- one symbolic representation maps to multiple images, that differ in terms of exact pixels and object location.
%Our modified Shapes task follows \citet{Havrylov2017} implementation, in this case with $k=3$ distractors. 
%We artificially generate images in the same way as in the original Shapes dataset, focusing here on different colors, size, shapes, and positions.
%The generated images are 30 by 30 pixels, and some examples can be seen in Figure \ref{fig:shapes}.
%Following the experiment setup in \citet{Havrylov2017}, 
We use 80k, 8k, 40k images for train, validation and test sets, respectively.
Some example images are depicted in Figure \ref{fig:shapes}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{images/shapes_task}
	\caption{The modified Shapes task consists of showing an image the sender, and then letting the receiver deduce from the sender's message which image out of the target and $k$ distractors is the correct one.}
	\label{fig:shapes}
\end{figure}
 
We pre-train a CNN feature extractor for the images in a two-agent setting of the task (see Appendix \ref{sec:features} for more details). 
%The convolution layer architecture used to extract the features is similar to that in \citet{Choi2018}, where the image extraction is part of the agent model (see appendix \ref{sec:features} for more detail).


\subsection{Architecture and Training}

For our co-evolution experiments, we use the DARTS search space as described above.
For all cultural evolution approaches, we use an LSTM \cite{lstm} for both the sender and receiver architecture (see Appendix \ref{sec:agent_architecture} for more details).
%Unless otherwise specified, we use the same sizes and hyper-parameters for all models.
The sender and receiver models have a hidden size of 64 for the recurrent layer and an embedding layer of size 64. 
Further, we use a vocabulary size $V$ of 4, with an additional bound token serving as the indicator for beginning and end-of-sequence. 
We limit the maximum length of a sentence $L$ to 5. \footnote{The values for $V$ and $L$ were picked to provide a strong communication bottleneck to promote the emergence of structured and compressed languages, following the intuitions from \citet{Kottur2017} that natural language patterns do not emerge `naturally'.}

We back-propagate gradients through the discrete step outputs (message) of the sender by using the Straight-Through (ST) Gumbel-Softmax Estimator \citep{gumbel}.
We run all experiments with a fixed temperature $\tau=1.2$.
%where decreasing $\tau$ (approaching 0) reproduces the effect of an $argmax$, and increasing $\tau$ (approaching 10) converges to a uniform distribution over the vocabulary set.  
We use the default Pytorch \cite{paszke2017automatic} Adam \cite{adam} optimiser with a learning rate of 0.001 and a batch-size of 1024.
Note that the optimiser is reset for every batch.

% multi-agent settings
For all multi-agent experiments we use a population size of 16 senders and 16 receivers. 
%Note that this is significantly more than \citet{Cogswell2019}, who uses a population of only 5 Q-bots and 5 A-bots.
The culling rate $\alpha$ is set to $0.25$ or four agents, and we cull (re-initialise or mutate) every $l=5k$ iterations.
We run the experiments for a total of $I=500k$ iterations, and evaluate the populations before each culling step. 
%During evaluation on the validation set, a random receiver is selected and all 

%The sender and receiver architectures are further described in Appendix , and, apart from switching the RNN LSTM with an evolved cell, their internal processes remain fixed through our experiments. 

\subsection{Evaluation}
 
We use an range of metrics to evaluate both the population of agents and the emerging languages.

% \subsubsection{Language related metrics}

\paragraph{Jaccard Similarity} We measure the consistency of the emerged languages throughout the population using \textit{Jaccard Similarity}, which is defined as the ratio between the size of the intersection and the union of two sets.
We sample $200$ messages per input image for each possible sender-receiver pair and average the Jaccard Similarity of the samples over the population. 
A high Jaccard Similarity between two messages is an indication that the same tokens are used in both messages. 
% TODO: give reference where else this was used?

\paragraph{Proportion of Unique Matches}
We compute how similar the messages that different agents emit for the same inputs by looking at all possible (sender, message) pairs for one input and assess whether they are the same.
This metric is 1 when all agents always emit the same messages for the same inputs.

\paragraph{Number of Unique Messages}
We compute the average \textit{number of unique messages} generated by each sender in the population.
An intuitive reference point for this metric is the number of images with distinct symbolic representations.
If agents generate more messages than expected by this reference point, this demonstrates that they use multiple messages for the images that are -- from a task perspective -- identical.
%A smaller number of unique messages, on the other hand, indicates that the agent is using a simpler language which is underspecified compared to the symbolic description of the image.

\paragraph{Topographic Similarity} Topographic similarity, used in a similar context by \citet{lazaridou2018emergence}, represents the similarity between the meaning space (defined by the symbolic representations) and the signal space (the messages sent by an agent).
It is defined as the correlation between the distances between pairs in meaning space and the distances between the corresponding messages in the signal space.
We compute the topographic similarity for an agent by sampling 5,000 pairs of symbolic inputs and corresponding messages and compute the Pearson's $\rho$ correlation between the cosine similarity of the one-hot encoded symbolic input pairs and the cosine similarity of the one-hot encoded message pairs.

% \subsection{Agent related metrics}

\paragraph{Average Population Convergence} To estimate the speed of learning of the agents in the population, estimate the \textit{average population convergence}.
For each agent, at each point in time, this is defined as the agents average performance from the time it was born until it had the age of the current youngest agent in the population (analogous to the fitness criterion defined in Section~\ref{sec:fitness}).
To get the average population convergence, we take we average those values for all agents in the population.

\paragraph{Average Agent Entropy} We compute the average certainty of sender agents in their generation process by computing and averaging their \textit{entropy} during generation.


%Since this is a correlation coefficient, its maximum value is 1 and happens when the messages exactly model the symbolic representation. 
%\textcolor{gray}{Note that our implementation differs slightly from  \citet{topographic}, who uses the Levenshtein (edit distance) as a measure of similarity for signals.}


% \begin{itemize}
% \item \textbf{Average Population Convergence}: This is the convergence metric as defined in section \ref{sec:fitness}, averaged over all senders and receivers.
% \item \textbf{Average Agent Entropy}: It is given by the average sender's entropy during generation and describes the certainty of the agents in their generation process.

% \item \textbf{Jaccard Similarity}: 
%\item \textcolor{gray}{Also known as Intersection over Union (IoU), 
% It is defined as the size of the intersection over the size of the union of two sets (in this case - messages). 
% We sample $200$ messages for each possible pair of senders and average the Jaccard Similarity of the samples over the population. 
% A high Jaccard Similarity between two messages is an indication that the same tokens are used in both messages. 
%\textcolor{gray}{While Jaccard Similarity does not retain order, in general the higher the average Jaccard Similarity between the sampled messages of two agents, the closer their language.}

% \item \textbf{Proportion of Unique Matches}: Looks at all possible pairs of senders and their messages and measures the average number of times a message is the same. 
% This metric is 1 when all agents always emit the same messages for the same inputs.
% 
% \item \textbf{Number of Unique Messages}: Represents the number of unique messages generated by each sender agent averaged over the population. A small number of unique messages would indicate a simpler language.
% A high number of unique messages would indicate a more specialised and complex language, whereas a small number would indicate a simpler language (assuming a comparable accuracy on the task). 
%\textcolor{gray}{Note that if agents do not use many unique  sentences to represent objects, this does not necessarily mean that their solution is more compositional, structured or abstract than otherwise, since a group of agents that emit always the same message regardless of input would score low on the number of unique messages. 
%Which is why the quality of these messages and task success of the agents should also be scrutinised along with this metric to provide context. } 

% \item \textbf{Topographic Similarity}:  Represents the correlation of the similarity between pairs of meanings (symbolic representation) and corresponding pairs of signals (messages). 
% For each agent, we sample 5,000 pairs of symbolic inputs and the corresponding messages outputted by the agent, and find the Pearson's $\rho$ correlation between the cosine similarity of the one-hot encoded symbolic input pairs and the cosine similarity of the one-hot encoded message pairs.
% %Since this is a correlation coefficient, its maximum value is 1 and happens when the messages exactly model the symbolic representation. 
% %\textcolor{gray}{Note that our implementation differs slightly from  \citet{topographic}, who uses the Levenshtein (edit distance) as a measure of similarity for signals.}
% 
% \end{itemize}

% While convergence depends on training loss, since it is a measure of how fast an agent learns, all other metrics reported in this paper are obtained by running the models on the validation set. 






==> evolving_networks copy/intro2.tex <==
\section{Introduction}
Human languages show a remarkable degree of structure and complexity.
In the evolution of this complex structure, several different intertwined \emph{pressures} are assumed to have played a role.
The first of this pressures concerns the function of language: as language is used co communicate, it should allow effective communication between proficient language users \citep[e.g.][]{Smith2012}. 
The pressure that this forms on the shape of language is strongly intertwined with the nature of the proficient user: what features of language allow effective communication depends on the abilities of the user as well as what they want to communicate about.

A second pressure on the shape of human language stems from the fact that language must be \emph{learnable}.
Unlike animal languages, which are taken to be mostly innate, human languages must be re-acquired by each individual \cite{Pinker1990, Hurford99}.
A language can thus only survive it can successfully be transmitted to a next generation of learners.
In the field of language evolution, this transmission process is referred to with the name \emph{cultural evolution}, while the process of change that occurs as a consequence is called \emph{cultural evolution}.

Also this learnability pressure is intertwined with the language user: What is learnable depends on the inductive biases of the learner.

The importance of cultural evolution for the emergence of structure is supported by a number of artificial language learning studies \citep[e.g.][]{Saldana2018} and computational studies using the Iterated Learning paradigm, in which agents learn a language by observing the output produced by another agent from the previous `generation' \citep[e.g.][]{kalish2007,kirby2008,Kirby2015}.

3. While all of these components are assumed to be important for the shape of human language, how communication, cultural evolution and the learning biases of the (human) learner interact with each other and influence the structure of human language is largely unknown.

4. Computationally, the emergence of language can be studied by simulating it in (populations of) artificial agents, and investigating the structure, level of compositionality and morphosyntactic properties of the resulting languages \citep{Kirby2001, Kirby2002}.
Originally, such work was based on logic and symbolic representations \cite{Kirby2001, Christiansen2003}, but with the advent of modern deep learning methods and sequence-to-sequence models \cite{Sutskever2014}, there has been a renewed interest in simulating the emergence of language through neural network agents \citep[i.a.][]{Lazaridou2016,Havrylov2017}.
Such work typically involve the use of \emph{referential games} \citep{lewis1969convention}, in which two or more agents have to emerge a language to refer to a shared set of images.
These studies are thus motivated by the second constraint -- that language is used to communicate -- but do not consider the second constraint which is imposed by the transmission bottleneck that arises as a consequence of cultural transmission nor the impact of the learning biases of the artificial agents itself, which are inextricably connected.

In a recent study, \cite{Cogswell2019} proposed a method to include cultural evolution in a language emergence game, by simulating a large population of agents and pairing them randomly to solve a referential game.
This approach is more naturally aligned with pressures in humans language evolution \citep[see e.g.][]{Wray2007}, but fails to account for the  fact that cultural evolution and the learning biases of the artificial agents are two sides of the same coin: what language is learnable depends on the learning biases of the learner.
If the artificial agent is not suitable to solve the task at hand through communication, they will -- at best -- converge to a language that doesn't allow for effective communication or is difficult to learn for every new agent or -- at worst -- not converge to an appropriate culturally transmittable language at all.

In this paper, we will therefore to integrate the three components described above, and setup a framework in which their interaction can be studied.
This framework, which we refer to with the term \ourframework, consists of \emph{a referential game}, played by \emph{a changing population of agents} -- simulating cultural evolution -- which are subject to \emph{architectural evolution}, allowing them to \emph{co-evolve} with the language.

Our contributions are three-fold fold:
\vspace{-2mm}\begin{itemize}\setlength{\itemsep}{-1mm}
        \item We introduce the \textit{\ourframework}, that allows to model both cultural and architectural evolution in a population of agents;
        \item We collect a large number of tests from previous work and combine them into an extensive test suits for language emergence games;
        \item We demonstrate that emerging languages benefit from including cultural transmission \emph{as well as} architectural evolution, but the best results are achieved when languages and agents can co-evolve.
\end{itemize}

In the remainder of this paper, we ... \dieuwke{add..}
%To model genetic evolution, we explore that space of different architectures using [darts].
% We show how networks provided with genetic and cultural evolution combined are the quickest to learn the language and the most effective to communicate.

% Recently, there has been a lot of buzz about neural networks not capable of compositionality. However, this is not big surprise if we consider that we do not provide them with the same transmission pressures and adaptation capabilities. 

% In this paper, we investigate the impact of cultural and genetic adaptation on cultural transmission in neural networks tasked with grounded communication.

% in facilitating cross-generational transmission. 
% To model culturual adapatation we bla bla [cite batra]. To model genetic evolution, we explore that space of different architectures using [darts].
%As for genetic adaptation, using neuroevolution we explore the space of different architectures in search of architectural properties that make networks faster in learning a language [cite darts]. 
% We show how networks provided with genetic and cultural evolution combined are the quickest to learn the language and the most effective to communicate.

%We embed genetic evolution in a more general linguistic evolution framework that models also the cultural evolution of language. This allows us to weigh the contribution of the two types of adaptation in fitting the cross-generational transmission pressures. 

% The closest to our contribution is the work by [cite batra], but we differ from them for two key differences. First, while they focus only on cultural adaptation of language, we incorporate also genetic adaptation, offering a more complete evolution dynamics. 
% fit the cross-generational transmission pressures best,  is crucial to reach an optimal
%This allows us to weigh the contribution of the two types of adaptation in fitting the cross-generational transmission pressures. 
% Second, we present networks with real images instead of symbolic input, which is not only cognitive more plausible, but it also brings us closer to the development of artificial agents that can communicate in the real world.  
%In this paper, we study the emergence of compositional language in the context of genetic evolution of traits underlying interactive communication. 

%Using neuroevolution, we explore the space of different architectures in search of architectural properties that make networks more suitable to learn and use language.
%
%We embed genetic evolution in a more general linguistic evolution framework that models also the cultural evolution of language. This allows us to weigh the contribution of cultural and genetic adaptations. 




%the evolution of language in the context of the biological evolution of the necessary traits to support a successful communicative interaction. 
%
%Unlike animal languages, which are taken to be mostly innate, human languages require a good equilibrium between where each individual starts from a powerful genetic predisposition but has nonetheless to re-acquire
%
%
%According to evolutionary linguistics, \emph{compositionality makes the language simpler to transmit across generations while preserving communication efficiency} [cite]. 

%
%Computational simulations using iterated learning techniques have shown that transmission pressures indeed encourage virtual agents to develop compositional languages [cite]. However, in all these studies, researchers have presented learners with inputs in hand-engineered, symbolic formats rather than raw perceptual inputs as humans receive. This approach is not only cognitive implausible, but it also hinders the development of artificial agents that can communicate in the real world. Further, such simulations have focused only on cultural adaptations given the transmission pressure, forgetting about genetic adaptation. 
%
%Lately, numerous models of grounded communication have been proposed to move from symbolic to raw inputs [cite]. This represents important progress towards the development of more realistic dialogue agents. However, none of them incorporate forms of cultural or phylogenetic adaptation and therefore tend to produce holistic, unstructured languages [cite].
%
%
%Here, we study whether compositional abilities to communicate about raw visual input can be the result of the coevolution of cultural language transmission pressures and biological evolution of traits that support communication. 

%In this paper, we introduce cultural and neuroevolution in virtual agents that communicate about raw visual input to give rise to compositional structures in their language. 



==> evolving_networks copy/introduction.tex <==
\section{Introduction}
Human languages show a remarkable degree of structure and complexity.
In the evolution of this complex structure, several different intertwined \emph{pressures} are assumed to have played a role.
The first of these pressures concerns the function of language: as language is to communicate, it should allow effective communication between proficient language users \citep[e.g.][]{Smith2012}. 
This pressure is strongly intertwined with the nature of the proficient user: what features of language allow effective communication depends
on the abilities of the user to use the language.
%on the abilities of the user as well as what they want to communicate about.

A second pressure on the shape of human language stems from the fact that language must be \emph{learnable}.
Unlike animal languages, which are taken to be mostly innate, human languages must be re-acquired by each 
individual \cite{Pinker1990, Hurford99}.
A language can only survive if it can successfully be transmitted to a next generation of learners.
In the field of language evolution, this transmission process is referred to as \emph{cultural transmission}, while the process of change that occurs as a consequence is called \emph{cultural evolution}.\footnote{The importance of cultural evolution for the emergence of structure is supported by a number of artificial language learning studies \citep[e.g.][]{Saldana2018} and computational studies using the Iterated Learning paradigm, in which agents learn a language by observing the output produced by another agent from the previous `generation' \citep[e.g.][]{kalish2007,kirby2008,Kirby2015}.}
Like the pressures arising from the function of language, the way that cultural evolution shapes language also depends on the language users: what is learnable depends on the inductive biases of the learner.
% In this paper,  ...
% 3. While all of these components are assumed to be important for the shape of human language, how communication, cultural evolution and the learning biases of the (human) learner interact with each other and influence the structure of human language is largely unknown.


Computationally, the emergence of language can be studied through simulation with artificial agents and by investigating the resulting languages for structure, level of compositionality, and morphosyntactic properties \citep{Kirby2001, Kirby2002}.
Originally based on logic and symbolic representations \cite{Kirby2001, Christiansen2003}, with the advent of modern deep learning methods, there has been a renewed interest in simulating the emergence of language through neural network agents \citep[i.a.][]{Lazaridou2016,Havrylov2017}.
Such work typically involves the use of \emph{referential games} \citep{lewis1969convention}, in which two or more agents have to emerge a language to obtain a shared reward.

%These studies are thus motivated by the first constraint -- that language is used to communicate -- but do not consider the second constraint which is imposed by the transmission bottleneck that arises as a consequence of cultural transmission nor the impact of the learning biases of the artificial agents itself, which are inextricably connected.
These studies are motivated by the first pressure:  language as a tool for effective communication. 
However, they fail to consider the second pressure: language must be learnable by new agents.
They also fail to study the impact of the learning biases of the artificial agents themselves, which underlies both pressures.
In a recent study, \citet{Cogswell2019} proposed a method to include cultural evolution in a language emergence game. % , by simulating a large population of agents and pairing them randomly to solve a referential game.
Their approach is more naturally aligned with pressures in humans language evolution than single agent referential games \citep[see e.g.][]{Wray2007}, but fails to account for the fact that cultural evolution and the learning biases of the artificial agents are two sides of the same coin: what language is learnable depends on the learning biases of the learner.
%If the artificial agent is not suitable to solve the task at hand through communication, they will -- at best -- converge to a language that doesn't allow for effective communication or is difficult to learn for every new agent or -- at worst -- not converge to an appropriate culturally transmittable language at all.

In this paper, we will therefore integrate the three components described above -- communication, cultural evolution and learning biases --  and setup a framework in which their interaction can be studied.
This framework, which we refer to with the term \ourframework, consists of \emph{a referential game}, played by \emph{a changing population of agents} -- simulating cultural evolution -- which are subject to \emph{architectural evolution} -- simulating the learning biases of the learners and allowing them to \emph{co-evolve} with the language.

Our contributions are three-fold fold:
\vspace{-2mm}\begin{itemize}\setlength{\itemsep}{-1mm}
        \item We introduce the \textit{\ourframework}, that allows to model both cultural and architectural evolution in a population of agents;
        \item We collect a large number of tests from previous work and combine them into an extensive test suits for language emergence games;
        \item We demonstrate that emerging languages benefit from including cultural transmission \emph{as well as} architectural evolution, but the best results are achieved when languages and agents can co-evolve.
\end{itemize}

%In the remainder of this paper, we ... \dieuwke{add..}
%To model genetic evolution, we explore that space of different architectures using [darts].
% We show how networks provided with genetic and cultural evolution combined are the quickest to learn the language and the most effective to communicate.

% Recently, there has been a lot of buzz about neural networks not capable of compositionality. However, this is not big surprise if we consider that we do not provide them with the same transmission pressures and adaptation capabilities. 

% In this paper, we investigate the impact of cultural and genetic adaptation on cultural transmission in neural networks tasked with grounded communication.

% in facilitating cross-generational transmission. 
% To model culturual adapatation we bla bla [cite batra]. To model genetic evolution, we explore that space of different architectures using [darts].
%As for genetic adaptation, using neuroevolution we explore the space of different architectures in search of architectural properties that make networks faster in learning a language [cite darts]. 
% We show how networks provided with genetic and cultural evolution combined are the quickest to learn the language and the most effective to communicate.

%We embed genetic evolution in a more general linguistic evolution framework that models also the cultural evolution of language. This allows us to weigh the contribution of the two types of adaptation in fitting the cross-generational transmission pressures. 

% The closest to our contribution is the work by [cite batra], but we differ from them for two key differences. First, while they focus only on cultural adaptation of language, we incorporate also genetic adaptation, offering a more complete evolution dynamics. 
% fit the cross-generational transmission pressures best,  is crucial to reach an optimal
%This allows us to weigh the contribution of the two types of adaptation in fitting the cross-generational transmission pressures. 
% Second, we present networks with real images instead of symbolic input, which is not only cognitive more plausible, but it also brings us closer to the development of artificial agents that can communicate in the real world.  
%In this paper, we study the emergence of compositional language in the context of genetic evolution of traits underlying interactive communication. 

%Using neuroevolution, we explore the space of different architectures in search of architectural properties that make networks more suitable to learn and use language.
%
%We embed genetic evolution in a more general linguistic evolution framework that models also the cultural evolution of language. This allows us to weigh the contribution of cultural and genetic adaptations. 




%the evolution of language in the context of the biological evolution of the necessary traits to support a successful communicative interaction. 
%
%Unlike animal languages, which are taken to be mostly innate, human languages require a good equilibrium between where each individual starts from a powerful genetic predisposition but has nonetheless to re-acquire
%
%
%According to evolutionary linguistics, \emph{compositionality makes the language simpler to transmit across generations while preserving communication efficiency} [cite]. 

%
%Computational simulations using iterated learning techniques have shown that transmission pressures indeed encourage virtual agents to develop compositional languages [cite]. However, in all these studies, researchers have presented learners with inputs in hand-engineered, symbolic formats rather than raw perceptual inputs as humans receive. This approach is not only cognitive implausible, but it also hinders the development of artificial agents that can communicate in the real world. Further, such simulations have focused only on cultural adaptations given the transmission pressure, forgetting about genetic adaptation. 
%
%Lately, numerous models of grounded communication have been proposed to move from symbolic to raw inputs [cite]. This represents important progress towards the development of more realistic dialogue agents. However, none of them incorporate forms of cultural or phylogenetic adaptation and therefore tend to produce holistic, unstructured languages [cite].
%
%
%Here, we study whether compositional abilities to communicate about raw visual input can be the result of the coevolution of cultural language transmission pressures and biological evolution of traits that support communication. 

%In this paper, we introduce cultural and neuroevolution in virtual agents that communicate about raw visual input to give rise to compositional structures in their language. 



==> evolving_networks copy/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

%\dieuwke{Here, we write:\begin{itemize}
%    \item A brief introduction to language emergence games (a bit like it is here now, but we should  double check also with the introduction
%    \item Some review of the results (in terms of structure mostly). Basically like the last few sentences in this paragraph, but a bit more %extensive
%    \item Some work that has been done on improving this (actually, the last ones can be cited also here, but also cogswell
%\end{itemize}gi
%I left the text below to take as guidance for rewriting this}
%
%\gautier{needs review - esp last paragraph which is too long}

%language emergence history
Much work has been done on the emergence of language in artificial agents and investigating its subsequent structure, compositionality and morphosyntax \cite{Kirby2001, Kirby2002}.
Originally, such work was based on logic and symbolic representations \cite{Kirby2001, Christiansen2003}, but with the advent of modern deep learning \cite{lecun2015deep}, there has been a renewed interest in simulating the emergence of language through neural network agents \citep[i.a.][]{Foerster2016,Kottur2017,Choi2018,Lazaridou2016,Havrylov2017,Mordatch2017}. In the exploration of language emergence, different training approaches and tasks have been proposed to encourage agents to learn and develop communication. 
In a typical setup, two players aim to develop a communication protocol in which one agent must communicate information it has access to (typically an image), while the other must guess it out of a line-up \citep{Evtimova2017,Lazaridou2016}.
%These tasks are commonly set up in an end-to-end setting where reinforcement learning can be applied. % and require communication to be solved in the optimal manner \cite{Lazaridou2016,Foerster2016, Kottur2017}.
%bottle necks

\citet{Kottur2017} show that `natural' language does not arise naturally in these communication games and it has to be incentivised by imposing specific restrictions on games and agents.
\citet{Havrylov2017} first demonstrated that using straight-through estimators were more effective than reinforcement learning in a collaborative task, and that optimizing rewards can lead to structured protocols (i.e. strings of symbols) to be induced from scratch. 
\citet{Mordatch2017} find that syntactic structure emerges in the  stream  of  symbol  uttered  by  agents, where symbols and syntax can be mapped to specific meanings or instructions. 
%They also find that agents settle on using a consistent sets of symbols for each meaning and avoid synonyms due to introducing a soft penalty on vocabulary size.
\citet{Choi2018} use qualitative analysis, visualization and a zero-shot test, to show that a language with compositional properties can emerge from environmental pressures.
%They measure message distinctness, Jaccard similarity, and agent perplexity over time and observe that consistent and similar messages emerge to describe the same meaning space.

\citet{chaabouni-etal-2019-word} find that emerged languages, unlike human languages, do not naturally prefer non-redundant encodings. 
\citet{chaabouni2020compositionality} further find that while generalization capabilities can be found in the languages, compositionality itself does not arise from simple generalization pressures.
\cite{rodriguez-luna-etal-2020-internal} encourage desirable properties of human languages, such as compositionality, to emerge through well-crafted auxiliary pressures.
Finally, \citet{harding-graesser-etal-2019-emergent} demonstrate with experiments on populations of agents that language can evolve and simplify through the interactions of different communities.


% Population / Resetting based approaches
%Recent works by \citet{Cogswell2019} and others use population of agents $N>2$ and periodic resetting to create additional environmental pressures onto emerging languages.
\citet{Cogswell2019} build upon the emergent language research by introducing cultural transmission as a pressure in referential games. 
They use a pool of agents with a resetting mechanism and show that this further encourages the emerging language to display compositional properties and structure allowing it to generalize better.
Pairing agents with one another in a larger population setting introduces cultural evolution, but it is the pressure introduced by the partial resetting which forces remaining agents to emerge a language that is quickly learnable by a new agent. While \citet{Cogswell2019} is the most related work to ours, an important difference is that they focus on cultural evolution only, without taking into account the learning biases of the agents via modelling architectural evolution.

% In the name of space, we have to sacrifice something
%\citet{li2019easeofteaching} analyse language structure in a population setting and find that periodic resetting leads to easier to learn languages.
%\citet{tieleman2019shaping} introduce community-based auto-encoders and find that increasing community size leads to better learned representations.
%\citet{ren2020compositional} introduce neural iterated learning (NIL) in which they reset two agents periodically to pressure language towards compositional structure.
%They show that compositional languages (high topological similarity) are easier to learn and provide advantages for generalization.


% For instance, if the task allows agents to communicate an unlimited number of times with no negative impact then the agents could simply transmit the data with no real compression or emergence of language.


==> evolving_networks copy/related_work_old.tex <==
\section{Related Work}
\label{sec:related_work}


\subsection{Language Emergence}
\label{subsec:language_emergence}
%[max one column with approx 10/15] 

%language emergence history
\textcolor{gray}{Much work has been done on the emergence of language in artificial agents and investigating its subsequent structure, compositionality and morphosyntax \cite{Kirby2001, Kirby2002}.} 
\textcolor{gray}{The original computer simulations dealt with symbolic logic and representations \cite{Kirby2001, Christiansen2003}, but with the advent of modern deep learning methods and sequence-to-sequence models \cite{Sutskever2014}, there has been a renewed interest in simulating the emergence of language through neural network agents \cite{Foerster2016,Kottur2017,Choi2018,Lazaridou2016,Havrylov2017,Mordatch2017}. }

%setting
In the exploration of language emergence, different training approaches and tasks have been proposed in order to encourage agents to learn and develop communication. 
These tasks are commonly set up in an end-to-end setting where reinforcement learning can be applied, and require communication to be solved in the optimal manner \cite{Lazaridou2016,Foerster2016, Kottur2017}.
This is often a two-player referential game where one agent must communicate the information it has access to (typically an image), while the other must guess it out of a lineup \cite{Evtimova2017,Lazaridou2016}.
%bottle necks
Even in a two-player dialogue game, \citet{Kottur2017} have shown that `natural language' does not naturally arise, and agents must still be incentivised and forced to communicate through bottlenecks and intelligent design.
For instance, if the task allows agents to communicate an unlimited number of times with no negative impact then the agents could simply transmit the data with no real compression or emergence of language.

%RL vs gumbel softmax
% could add that cannot backprop gradients in traditional RL setting
\textcolor{gray}{Additionally, since reinforcement learning environments are computationally expensive, \citet{Havrylov2017} suggest using the Gumbel-Softmax trick to back-propagate gradients through the sender's discrete communication outputs.}

%compositionality?
\textcolor{gray}{Even when the task is not grounded in human language, it has been found that structure and some compositionality arises from the emerged language \cite{Mordatch2017, Choi2018}.
The structure and `compositionality' of the emerged languages is important to their success since a non-structured random language would poorly convey information and negatively impact task success.
So even though an accurate measurement for the degree of compositionality remains an unsolved problem \cite{Andreas2019, Lowe2019}, task success is still a strong indicator that the language is useful.}


\subsection{Cultural and Genetic Language Evolution}
%[max one column with approx 10]
% cultural vs biological
Language is often viewed as an inherently new human faculty, yet individual languages continue to evolve considerably within its framework \cite{Bolhuis2014}.
This evolution of language in humans can be seen as partly caused by cultural transmission, and the process of cultural evolution.
\citet{Christiansen2003} assert that the question of biological versus cultural evolution in the origin of language is complex, and that it ultimately arises `from three distinct but interacting adaptive systems: individual learning, cultural transmission, and biological evolution'.
This cultural evolution process is thought to also force structure and a certain compression onto language, since a language must be used by all the individuals of the society (culture) in which it resides and still be suitable for a variety of tasks.
\citet{Kirby2015} define those two pressures as compressibility and expressivity and finds that structure arises from the trade-off between these pressures in generated languages.
These findings were further reinforced in artificial human studies by \citet{Saldana2018}, which provided evidence that cultural transmission allows compositional hierarchical structure to emerge in language.
%Thus the advantage to bringing such a cultural pressure to an artificial setting, is that not only is it plausibly explainable as a source of compositionality in human language, it should also translate to higher compositionality and simpler structured generated languages. 

\subsection{Cultural evolution of language}
To simulate cultural evolution and transmission pressure, the process of Iterated Learning has been used in the past with success \cite{KALISH2007,Kirby2008,Kirby2015}. 
Iterated learning is the process where an agent learns by observing the output produced by another agent that preceded it \cite{KALISH2007}.
Effectively, this can done by training an agent on a subset of the data, doing inference on the full set, and subsequently using a new subset of the produced inferences as a new training data. 
Iterating over this process forces the agent to evolve its language over time by changing the available training examples, and thus pressuring the agent to produce a language which is general enough in order to perform well on unseen data. 

%Population based Cultural evolution
As recently proposed by \citet{Cogswell2019}, an alternative way of imposing cultural pressures on an agent, is by simulating a large populations of them, and pairing them randomly to solve the task. 
Over time this should lead to the population developing a common language, assuming that the agents are randomly assigned to each other and are not given clues about which agents they are paired with. 
This approach is more naturally aligned with cultural pressures in humans, since instead of simulating the cultural pressure through single agent iterations, it is instead simulated through a larger population of agents and their individual interactions \cite{Dunbar1993,Wray2007}.
Recent cognitive experiments by \citet{Raviv2019} have also shown that compositional languages can emerge in small human groups from the pressure of multiple interaction partners and an expanding meaning space.
This population based approach to cultural pressure is used in this paper.


\subsection{Evolving neural networks}
%[max one column with approx 10] 
However, as \citet{Christiansen2003} outline, cultural evolution and transmission pressures are not enough to explain the origin of language and we must also consider the biological evolution process that has endowed humans with the capabilities for it.

%traditional NAS
Traditional phylogenetic evolution techniques in neural networks have a long history in evolutionary computation since the 1980s. 
Neural Architectural Search (NAS) focuses on searching the architecture space of the networks, unlike many traditional evolutionary techniques which often include parameter weights in their search space.
Some of the earlier techniques such as NEAT gained considerable traction as a sound way of doing topology search using biologically inspired concepts \cite{Stanley2002}.
NAS methods however have mostly reverted to optimising solely the neural architecture and using gradient based methods such as SGD for weight optimisation due to the large parameter space of modern architectures (see, e.g., \citet{Elsken2018} for a sruvey). 


%Gradient based NAS
More recently, state of the art one-shot search techniques such as ENAS (Efficient Neural Architecture Search) and DARTS (Differentiable Architecture Search) have allowed to bring a gradient-based approach to NAS through the use of intelligent weight-sharing schemes  \cite{Liu2018,Pham2018}.
ENAS uses a reinforcement learning approach to compute the gradients for the architecture controller, while DARTS train all possible architectures at the same time and alternates back-propagation between the network and architecture weights \cite{Liu2018}.
Further works by Cai et al. who use a path binarisation approach to weight-sharing, and Li et al. have also shown that it is not even necessary to train the entire space of architecture simultaneously and one can randomly sample over the space and still obtain state of the art results \cite{Cai2018,Li2019}.

%Our approach
%Still unsure here...
%Maybe weight sharing is too open 






==> evolving_networks copy/results.tex <==
\section{Results}
\label{sec:results}
%\dieuwke{Split in two sections: results and analysis. Some of the text directly below might need to go in the next section.}
%\gautier{Feels a bit weird to have such a short Results section - do we try to split more evenly between Results and Analysis?}

We now present a detailed comparison of our cultural and co-evolution setups.
For each approach, we averaged over four random seeds, the error bars in all plots represent the standard deviation across these four runs.
To analyse the evolution of both agents and languages, we consider the development of all previously outlined metrics over time.
We then test the best converged languages and architectures in a single sender-receiver setup, to assess the impact of cultural and genetic evolution more independently.
In these experiments, we compare also directly to a single sender-receiver baseline, which is impossible for most of the metrics we consider in this paper.
Finally, we briefly consider the emerged architectures from a qualitative perspective.

\subsection{Task performance}

We first confirm that all setups in fact converge to a solution to the task.
As can be seen in Figure \ref{fig:acc_loss}, all populations converge to a (close to perfect) solution to the game. %\footnote{For a plot of the development of accuracy over time, we refer to Appendix~\ref{sec:appendix_analysis}}
The \texttt{\normalsize cu-age} approach slightly outperforms the other approaches, with a accuracy that surpasses the $95\%$ accuracy mark.
Note that, due to the ever changing population, the accuracy at any point in time is an average of both `children' and `adults', that communicate with different members of the population. % and is thus difficult to compare with a single sender-receiver setup.

%results of running cultural evolution only and cultural/genetic co-evolution for 500k iterations and display the loss over time, as well as the accuracy at $i=500k$ (see Appendix \ref{sec:appendix_analysis} for a plot of accuracy over time).\footnote{Note that we do not include a two-agent  baseline when comparing against cultural evolution or the LTE since culling does not make it comparable.}
% For each approach, four random seeds were tried, and the error bar on the accuracy represents the standard deviation for each result. 
% We observe a slightly better end performance in some of the cultural evolution runs compared to co-evolution, the \textbf{age} selection policy surpasses the $95\%$ accuracy mark. 
%Over time, all models tend to converge to approximately the same accuracy with some variations caused by the stochasticity introduced in the culling process.
% However, accuracy at a certain time-step or even over time can be misleading when analysing the true impact of the LTE on the language and architecture of the agents. 
% At any point in time the population consists of both `children' and `adults', and the accuracy measure is an average of their performance. 

%The process itself relies on the pressure it applies to the population, therefore if a task is perfectly solved when agents are constantly being replaced, this would signify that either the pressure is not strong enough or the task too simple.

% need to fix this plot to make legible in text (not sure if there is space to keep grouped)
\begin{figure}[!h]
		% \begin{subfigure}{\columnwidth}
		\includegraphics[width=\columnwidth, trim=20mm 0 20mm 10mm, clip]{images/run_images/acc_bar}\hfill
	% \end{subfigure}
	\centering
	\caption{Average Population Accuracy of final populations.}
	\label{fig:acc_loss}
\end{figure}



==> evolving_networks copy/text_related_work_prev_stored.tex <==

\subsection{Evolution of Language}
%[max one column with approx 10]
% cultural vs biological
The evolution of human language is a well-studied but still poorly understood topic.
% Language is often viewed as an inherently new human faculty, yet individual languages continue to evolve considerably within its framework \cite{Bolhuis2014}.
% This evolution of language in humans can be seen as partly caused by cultural transmission, and the process of cultural evolution.
One particular open question concerns the relation between two different evolutionary processes: \textit{genetic} evolution of the agents in the population and \textit{cultural} evolution of the language itself \cite{fitch2010evolution}.
\citet{Christiansen2003} assert that the question of genetic versus cultural evolution ultimately arises from three distinct but interacting adaptive systems: individual learning, cultural transmission, and genetic evolution.

\subsubsection{Cultural Evolution}
Cultural transmission is thought to enforce structure and compression to languages, since a language must be used and learned by all individuals of the culture in which it resides and at the same time be suitable for a variety of tasks.
\citet{Kirby2015} define those two pressures as compressibility and expressivity and find that structure arises from the trade-off between these pressures in generated languages.
The importance of cultural evolution for the emergence of structure is supported by a number of artificial language learning studies \citep[e.g.][]{Saldana2018} and computational studies using the Iterated Learning paradigm, in which agents learn a language by observing the output produced by another agent from the previous `generation' \citep[e.g.][]{kalish2007,kirby2008,Kirby2015}.
An alternative way of imposing cultural pressures on agents, is by simulating a large population of them and pairing agents randomly to solve a communicative game \cite{Cogswell2019}.
This approach is more naturally aligned with cultural pressures in humans \citep[see e.g.][]{Wray2007} and is the one we use in this paper.
% since instead of simulating the cultural pressure through single agent iterations, it is instead simulated through a larger population of agents and their individual interactions \cite{Dunbar1993,Wray2007}.
% This population based approach to cultural pressure is used in this paper.

\subsubsection{Genetic Evolution}
While there is much controversy about the selection pressures under which the fundamental traits underlying the human ability to learn and use language evolved in other humans, that genetic evolution played an essential role in endowing humans with the capabilities to learn and use language is generally undebated.
Pre-modern humans, for instance, did not have the ability to speak or understand complex structures \citep{fitch2010evolution}.

There are several approaches to simulate genetic evolution of neural network agents.
%traditional NAS
%Traditional phylogenetic evolution techniques in neural networks have a long history in evolutionary computation since the 1980s. 
Neural Architectural Search (NAS) focuses on searching the architecture space of the networks, unlike many traditional evolutionary techniques which often include parameter weights in their search space.
Some of the earlier techniques such as NEAT gained considerable traction as a sound way of doing topology search using biologically inspired concepts \cite{Stanley2002}.
NAS methods however have mostly reverted to optimising solely the neural architecture and using gradient based methods such as SGD for weight optimisation due to the large parameter space of modern architectures (see, e.g., \citet{Elsken2018} for a survey). 


%Gradient based NAS
More recently, state-of-the-art one-shot search techniques such as ENAS (Efficient Neural Architecture Search) and DARTS (Differentiable Architecture Search) have allowed to bring a gradient-based approach to NAS through the use of intelligent weight-sharing schemes  \cite{Liu2018,Pham2018}.
%ENAS uses a reinforcement learning approach to compute the gradients for the architecture controller, while DARTS trains all possible architectures at the same time and alternates back-propagation between the network and architecture weights \cite{Liu2018}.
%Further works by \citet{Cai2018} who use a path binarisation approach to weight-sharing, and \citet{Li2019} have also shown that it is not even necessary to train the entire spaces of architectures simultaneously and that one can randomly sample over the space and still obtain state-of-the-art results.
In this work, we use the DARTS search space, which is constrained but still obtained state-of-the-art performance on benchmark natural language tasks \cite{Li2019}.

%Our approach
%Still unsure here...
%Maybe weight sharing is too open 






==> intro2.tex <==
\section{Introduction}
Human languages show a remarkable degree of structure and complexity.
In the evolution of this complex structure, several different intertwined \emph{pressures} are assumed to have played a role.
The first of this pressures concerns the function of language: as language is used co communicate, it should allow effective communication between proficient language users \citep[e.g.][]{Smith2012}. 
The pressure that this forms on the shape of language is strongly intertwined with the nature of the proficient user: what features of language allow effective communication depends on the abilities of the user as well as what they want to communicate about.

A second pressure on the shape of human language stems from the fact that language must be \emph{learnable}.
Unlike animal languages, which are taken to be mostly innate, human languages must be re-acquired by each individual \cite{Pinker1990, Hurford99}.
A language can thus only survive it can successfully be transmitted to a next generation of learners.
In the field of language evolution, this transmission process is referred to with the name \emph{cultural evolution}, while the process of change that occurs as a consequence is called \emph{cultural evolution}.

Also this learnability pressure is intertwined with the language user: What is learnable depends on the inductive biases of the learner.

The importance of cultural evolution for the emergence of structure is supported by a number of artificial language learning studies \citep[e.g.][]{Saldana2018} and computational studies using the Iterated Learning paradigm, in which agents learn a language by observing the output produced by another agent from the previous `generation' \citep[e.g.][]{kalish2007,kirby2008,Kirby2015}.

3. While all of these components are assumed to be important for the shape of human language, how communication, cultural evolution and the learning biases of the (human) learner interact with each other and influence the structure of human language is largely unknown.

4. Computationally, the emergence of language can be studied by simulating it in (populations of) artificial agents, and investigating the structure, level of compositionality and morphosyntactic properties of the resulting languages \citep{Kirby2001, Kirby2002}.
Originally, such work was based on logic and symbolic representations \cite{Kirby2001, Christiansen2003}, but with the advent of modern deep learning methods and sequence-to-sequence models \cite{Sutskever2014}, there has been a renewed interest in simulating the emergence of language through neural network agents \citep[i.a.][]{Lazaridou2016,Havrylov2017}.
Such work typically involve the use of \emph{referential games} \citep{lewis1969convention}, in which two or more agents have to emerge a language to refer to a shared set of images.
These studies are thus motivated by the second constraint -- that language is used to communicate -- but do not consider the second constraint which is imposed by the transmission bottleneck that arises as a consequence of cultural transmission nor the impact of the learning biases of the artificial agents itself, which are inextricably connected.

In a recent study, \cite{Cogswell2019} proposed a method to include cultural evolution in a language emergence game, by simulating a large population of agents and pairing them randomly to solve a referential game.
This approach is more naturally aligned with pressures in humans language evolution \citep[see e.g.][]{Wray2007}, but fails to account for the  fact that cultural evolution and the learning biases of the artificial agents are two sides of the same coin: what language is learnable depends on the learning biases of the learner.
If the artificial agent is not suitable to solve the task at hand through communication, they will -- at best -- converge to a language that doesn't allow for effective communication or is difficult to learn for every new agent or -- at worst -- not converge to an appropriate culturally transmittable language at all.

In this paper, we will therefore to integrate the three components described above, and setup a framework in which their interaction can be studied.
This framework, which we refer to with the term \ourframework, consists of \emph{a referential game}, played by \emph{a changing population of agents} -- simulating cultural evolution -- which are subject to \emph{architectural evolution}, allowing them to \emph{co-evolve} with the language.

Our contributions are three-fold fold:
\vspace{-2mm}\begin{itemize}\setlength{\itemsep}{-1mm}
        \item We introduce the \textit{\ourframework}, that allows to model both cultural and architectural evolution in a population of agents;
        \item We collect a large number of tests from previous work and combine them into an extensive test suits for language emergence games;
        \item We demonstrate that emerging languages benefit from including cultural transmission \emph{as well as} architectural evolution, but the best results are achieved when languages and agents can co-evolve.
\end{itemize}

In the remainder of this paper, we ... \dieuwke{add..}
%To model genetic evolution, we explore that space of different architectures using [darts].
% We show how networks provided with genetic and cultural evolution combined are the quickest to learn the language and the most effective to communicate.

% Recently, there has been a lot of buzz about neural networks not capable of compositionality. However, this is not big surprise if we consider that we do not provide them with the same transmission pressures and adaptation capabilities. 

% In this paper, we investigate the impact of cultural and genetic adaptation on cultural transmission in neural networks tasked with grounded communication.

% in facilitating cross-generational transmission. 
% To model culturual adapatation we bla bla [cite batra]. To model genetic evolution, we explore that space of different architectures using [darts].
%As for genetic adaptation, using neuroevolution we explore the space of different architectures in search of architectural properties that make networks faster in learning a language [cite darts]. 
% We show how networks provided with genetic and cultural evolution combined are the quickest to learn the language and the most effective to communicate.

%We embed genetic evolution in a more general linguistic evolution framework that models also the cultural evolution of language. This allows us to weigh the contribution of the two types of adaptation in fitting the cross-generational transmission pressures. 

% The closest to our contribution is the work by [cite batra], but we differ from them for two key differences. First, while they focus only on cultural adaptation of language, we incorporate also genetic adaptation, offering a more complete evolution dynamics. 
% fit the cross-generational transmission pressures best,  is crucial to reach an optimal
%This allows us to weigh the contribution of the two types of adaptation in fitting the cross-generational transmission pressures. 
% Second, we present networks with real images instead of symbolic input, which is not only cognitive more plausible, but it also brings us closer to the development of artificial agents that can communicate in the real world.  
%In this paper, we study the emergence of compositional language in the context of genetic evolution of traits underlying interactive communication. 

%Using neuroevolution, we explore the space of different architectures in search of architectural properties that make networks more suitable to learn and use language.
%
%We embed genetic evolution in a more general linguistic evolution framework that models also the cultural evolution of language. This allows us to weigh the contribution of cultural and genetic adaptations. 




%the evolution of language in the context of the biological evolution of the necessary traits to support a successful communicative interaction. 
%
%Unlike animal languages, which are taken to be mostly innate, human languages require a good equilibrium between where each individual starts from a powerful genetic predisposition but has nonetheless to re-acquire
%
%
%According to evolutionary linguistics, \emph{compositionality makes the language simpler to transmit across generations while preserving communication efficiency} [cite]. 

%
%Computational simulations using iterated learning techniques have shown that transmission pressures indeed encourage virtual agents to develop compositional languages [cite]. However, in all these studies, researchers have presented learners with inputs in hand-engineered, symbolic formats rather than raw perceptual inputs as humans receive. This approach is not only cognitive implausible, but it also hinders the development of artificial agents that can communicate in the real world. Further, such simulations have focused only on cultural adaptations given the transmission pressure, forgetting about genetic adaptation. 
%
%Lately, numerous models of grounded communication have been proposed to move from symbolic to raw inputs [cite]. This represents important progress towards the development of more realistic dialogue agents. However, none of them incorporate forms of cultural or phylogenetic adaptation and therefore tend to produce holistic, unstructured languages [cite].
%
%
%Here, we study whether compositional abilities to communicate about raw visual input can be the result of the coevolution of cultural language transmission pressures and biological evolution of traits that support communication. 

%In this paper, we introduce cultural and neuroevolution in virtual agents that communicate about raw visual input to give rise to compositional structures in their language. 



==> related_work_old.tex <==
\section{Related Work}
\label{sec:related_work}


\subsection{Language Emergence}
\label{subsec:language_emergence}
%[max one column with approx 10/15] 

%language emergence history
\textcolor{gray}{Much work has been done on the emergence of language in artificial agents and investigating its subsequent structure, compositionality and morphosyntax \cite{Kirby2001, Kirby2002}.} 
\textcolor{gray}{The original computer simulations dealt with symbolic logic and representations \cite{Kirby2001, Christiansen2003}, but with the advent of modern deep learning methods and sequence-to-sequence models \cite{Sutskever2014}, there has been a renewed interest in simulating the emergence of language through neural network agents \cite{Foerster2016,Kottur2017,Choi2018,Lazaridou2016,Havrylov2017,Mordatch2017}. }

%setting
In the exploration of language emergence, different training approaches and tasks have been proposed in order to encourage agents to learn and develop communication. 
These tasks are commonly set up in an end-to-end setting where reinforcement learning can be applied, and require communication to be solved in the optimal manner \cite{Lazaridou2016,Foerster2016, Kottur2017}.
This is often a two-player referential game where one agent must communicate the information it has access to (typically an image), while the other must guess it out of a lineup \cite{Evtimova2017,Lazaridou2016}.
%bottle necks
Even in a two-player dialogue game, \citet{Kottur2017} have shown that `natural language' does not naturally arise, and agents must still be incentivised and forced to communicate through bottlenecks and intelligent design.
For instance, if the task allows agents to communicate an unlimited number of times with no negative impact then the agents could simply transmit the data with no real compression or emergence of language.

%RL vs gumbel softmax
% could add that cannot backprop gradients in traditional RL setting
\textcolor{gray}{Additionally, since reinforcement learning environments are computationally expensive, \citet{Havrylov2017} suggest using the Gumbel-Softmax trick to back-propagate gradients through the sender's discrete communication outputs.}

%compositionality?
\textcolor{gray}{Even when the task is not grounded in human language, it has been found that structure and some compositionality arises from the emerged language \cite{Mordatch2017, Choi2018}.
The structure and `compositionality' of the emerged languages is important to their success since a non-structured random language would poorly convey information and negatively impact task success.
So even though an accurate measurement for the degree of compositionality remains an unsolved problem \cite{Andreas2019, Lowe2019}, task success is still a strong indicator that the language is useful.}


\subsection{Cultural and Genetic Language Evolution}
%[max one column with approx 10]
% cultural vs biological
Language is often viewed as an inherently new human faculty, yet individual languages continue to evolve considerably within its framework \cite{Bolhuis2014}.
This evolution of language in humans can be seen as partly caused by cultural transmission, and the process of cultural evolution.
\citet{Christiansen2003} assert that the question of biological versus cultural evolution in the origin of language is complex, and that it ultimately arises `from three distinct but interacting adaptive systems: individual learning, cultural transmission, and biological evolution'.
This cultural evolution process is thought to also force structure and a certain compression onto language, since a language must be used by all the individuals of the society (culture) in which it resides and still be suitable for a variety of tasks.
\citet{Kirby2015} define those two pressures as compressibility and expressivity and finds that structure arises from the trade-off between these pressures in generated languages.
These findings were further reinforced in artificial human studies by \citet{Saldana2018}, which provided evidence that cultural transmission allows compositional hierarchical structure to emerge in language.
%Thus the advantage to bringing such a cultural pressure to an artificial setting, is that not only is it plausibly explainable as a source of compositionality in human language, it should also translate to higher compositionality and simpler structured generated languages. 

\subsection{Cultural evolution of language}
To simulate cultural evolution and transmission pressure, the process of Iterated Learning has been used in the past with success \cite{KALISH2007,Kirby2008,Kirby2015}. 
Iterated learning is the process where an agent learns by observing the output produced by another agent that preceded it \cite{KALISH2007}.
Effectively, this can done by training an agent on a subset of the data, doing inference on the full set, and subsequently using a new subset of the produced inferences as a new training data. 
Iterating over this process forces the agent to evolve its language over time by changing the available training examples, and thus pressuring the agent to produce a language which is general enough in order to perform well on unseen data. 

%Population based Cultural evolution
As recently proposed by \citet{Cogswell2019}, an alternative way of imposing cultural pressures on an agent, is by simulating a large populations of them, and pairing them randomly to solve the task. 
Over time this should lead to the population developing a common language, assuming that the agents are randomly assigned to each other and are not given clues about which agents they are paired with. 
This approach is more naturally aligned with cultural pressures in humans, since instead of simulating the cultural pressure through single agent iterations, it is instead simulated through a larger population of agents and their individual interactions \cite{Dunbar1993,Wray2007}.
Recent cognitive experiments by \citet{Raviv2019} have also shown that compositional languages can emerge in small human groups from the pressure of multiple interaction partners and an expanding meaning space.
This population based approach to cultural pressure is used in this paper.


\subsection{Evolving neural networks}
%[max one column with approx 10] 
However, as \citet{Christiansen2003} outline, cultural evolution and transmission pressures are not enough to explain the origin of language and we must also consider the biological evolution process that has endowed humans with the capabilities for it.

%traditional NAS
Traditional phylogenetic evolution techniques in neural networks have a long history in evolutionary computation since the 1980s. 
Neural Architectural Search (NAS) focuses on searching the architecture space of the networks, unlike many traditional evolutionary techniques which often include parameter weights in their search space.
Some of the earlier techniques such as NEAT gained considerable traction as a sound way of doing topology search using biologically inspired concepts \cite{Stanley2002}.
NAS methods however have mostly reverted to optimising solely the neural architecture and using gradient based methods such as SGD for weight optimisation due to the large parameter space of modern architectures (see, e.g., \citet{Elsken2018} for a sruvey). 


%Gradient based NAS
More recently, state of the art one-shot search techniques such as ENAS (Efficient Neural Architecture Search) and DARTS (Differentiable Architecture Search) have allowed to bring a gradient-based approach to NAS through the use of intelligent weight-sharing schemes  \cite{Liu2018,Pham2018}.
ENAS uses a reinforcement learning approach to compute the gradients for the architecture controller, while DARTS train all possible architectures at the same time and alternates back-propagation between the network and architecture weights \cite{Liu2018}.
Further works by Cai et al. who use a path binarisation approach to weight-sharing, and Li et al. have also shown that it is not even necessary to train the entire space of architecture simultaneously and one can randomly sample over the space and still obtain state of the art results \cite{Cai2018,Li2019}.

%Our approach
%Still unsure here...
%Maybe weight sharing is too open 






==> text_related_work_prev_stored.tex <==

\subsection{Evolution of Language}
%[max one column with approx 10]
% cultural vs biological
The evolution of human language is a well-studied but still poorly understood topic.
% Language is often viewed as an inherently new human faculty, yet individual languages continue to evolve considerably within its framework \cite{Bolhuis2014}.
% This evolution of language in humans can be seen as partly caused by cultural transmission, and the process of cultural evolution.
One particular open question concerns the relation between two different evolutionary processes: \textit{genetic} evolution of the agents in the population and \textit{cultural} evolution of the language itself \cite{fitch2010evolution}.
\citet{Christiansen2003} assert that the question of genetic versus cultural evolution ultimately arises from three distinct but interacting adaptive systems: individual learning, cultural transmission, and genetic evolution.

\subsubsection{Cultural Evolution}
Cultural transmission is thought to enforce structure and compression to languages, since a language must be used and learned by all individuals of the culture in which it resides and at the same time be suitable for a variety of tasks.
\citet{Kirby2015} define those two pressures as compressibility and expressivity and find that structure arises from the trade-off between these pressures in generated languages.
The importance of cultural evolution for the emergence of structure is supported by a number of artificial language learning studies \citep[e.g.][]{Saldana2018} and computational studies using the Iterated Learning paradigm, in which agents learn a language by observing the output produced by another agent from the previous `generation' \citep[e.g.][]{kalish2007,kirby2008,Kirby2015}.
An alternative way of imposing cultural pressures on agents, is by simulating a large population of them and pairing agents randomly to solve a communicative game \cite{Cogswell2019}.
This approach is more naturally aligned with cultural pressures in humans \citep[see e.g.][]{Wray2007} and is the one we use in this paper.
% since instead of simulating the cultural pressure through single agent iterations, it is instead simulated through a larger population of agents and their individual interactions \cite{Dunbar1993,Wray2007}.
% This population based approach to cultural pressure is used in this paper.

\subsubsection{Genetic Evolution}
While there is much controversy about the selection pressures under which the fundamental traits underlying the human ability to learn and use language evolved in other humans, that genetic evolution played an essential role in endowing humans with the capabilities to learn and use language is generally undebated.
Pre-modern humans, for instance, did not have the ability to speak or understand complex structures \citep{fitch2010evolution}.

There are several approaches to simulate genetic evolution of neural network agents.
%traditional NAS
%Traditional phylogenetic evolution techniques in neural networks have a long history in evolutionary computation since the 1980s. 
Neural Architectural Search (NAS) focuses on searching the architecture space of the networks, unlike many traditional evolutionary techniques which often include parameter weights in their search space.
Some of the earlier techniques such as NEAT gained considerable traction as a sound way of doing topology search using biologically inspired concepts \cite{Stanley2002}.
NAS methods however have mostly reverted to optimising solely the neural architecture and using gradient based methods such as SGD for weight optimisation due to the large parameter space of modern architectures (see, e.g., \citet{Elsken2018} for a survey). 


%Gradient based NAS
More recently, state-of-the-art one-shot search techniques such as ENAS (Efficient Neural Architecture Search) and DARTS (Differentiable Architecture Search) have allowed to bring a gradient-based approach to NAS through the use of intelligent weight-sharing schemes  \cite{Liu2018,Pham2018}.
%ENAS uses a reinforcement learning approach to compute the gradients for the architecture controller, while DARTS trains all possible architectures at the same time and alternates back-propagation between the network and architecture weights \cite{Liu2018}.
%Further works by \citet{Cai2018} who use a path binarisation approach to weight-sharing, and \citet{Li2019} have also shown that it is not even necessary to train the entire spaces of architectures simultaneously and that one can randomly sample over the space and still obtain state-of-the-art results.
In this work, we use the DARTS search space, which is constrained but still obtained state-of-the-art performance on benchmark natural language tasks \cite{Li2019}.

%Our approach
%Still unsure here...
%Maybe weight sharing is too open 





